Denoising Pre-Training and Data Augmentation Strategies for Enhanced RDF Verbalization with Transformers

The task of verbalization of RDF triples has known a growth in popularity due to the rising ubiquity of Knowledge Bases (KBs). The formalism of RDF triples is a simple and efficient way to store facts at a large scale. However, its abstract representation makes it difficult for humans to interpret. For this purpose, the WebNLG challenge aims at promoting automated RDF-to-text generation. We propose to leverage pre-trainings from augmented data with the Transformer model using a data augmentation strategy. Our experiment results show a minimum relative increases of 3.73%, 126.05% and 88.16% in BLEU score for seen categories, unseen entities and unseen categories respectively over the standard training.

==> data/data.tex <==
\label{data_section}
We introduce in this section the different corpora utilized for both pre-training and fine-tuning.

\subsection{WebNLG Dataset}
\input{data/webnlg_data.tex}

\subsection{Data Augmentation}
\input{data/data_augmentation.tex}

==> table/results.tex <==
\begin{tabular}{c|c|c|c||cccc}
\hline
\textbf{WebNLG} & \textbf{WS1} & \textbf{ST1} & \textbf{CL} & \textbf{BLEU} & \textbf{METEOR} & \textbf{chrf++} & \multicolumn{1}{l}{\textbf{BLEURT}} \\ \hline
\multirow{3}{*}{\checkmark} & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{} & 55.24 & 0.401 & 0.680 & 0.56 \\
 &  &  &  & 12.9 & 0.167 & 0.319 & -0.62 \\
 &  &  &  & 11.17 & 0.162 & 0.310 & -0.64 \\ \hline
\multirow{3}{*}{\checkmark} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{} & \multirow{3}{*}{} & 57.3 & 0.417 & 0.701 & 0.58 \\
 &  &  &  & 29.16 & 0.301 & 0.518 & 0.1 \\
 &  &  &  & 21.02 & 0.265 & 0.452 & -0.06 \\ \hline
\multirow{3}{*}{\checkmark} & \multirow{3}{*}{} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{} & \textbf{59.32} & \textbf{0.428} & \underline{0.712} & \underline{0.6} \\
 &  &  &  & \textbf{35.77} & \textbf{0.326} & \textbf{0.565} & \textbf{0.26} \\
 &  &  &  & \underline{23.26} & \textbf{0.288} & \textbf{0.485} & \textbf{0.03} \\ \hline
\multirow{3}{*}{\checkmark} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{} & 57.49 & 0.420 & 0.702 & 0.59 \\
 &  &  &  & 32.33 & 0.310 & 0.535 & 0.18 \\
 &  &  &  & \textbf{23.42} & 0.275 & \underline{0.469} & \underline{-0.02} \\ \hline
\multirow{3}{*}{\checkmark} & \multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{\checkmark} & 54.78 & 0.399 & 0.676 & 0.56 \\
 &  &  &  & 11.94 & 0.156 & 0.295 & -0.68 \\
 &  &  &  & 12.45 & 0.156 & 0.298 & -0.63 \\ \hline
\multirow{3}{*}{\checkmark} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{} & \multirow{3}{*}{\checkmark} & 56.94 & 0.417 & 0.701 & 0.58 \\
 &  &  &  & 28.83 & 0.295 & 0.509 & 0.05 \\
 &  &  &  & 21.84 & 0.263 & 0.451 & -0.04 \\ \hline
\multirow{3}{*}{\checkmark} & \multirow{3}{*}{} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{\checkmark} & 58.36 & 0.422 & 0.703 & \textbf{0.61} \\
 &  &  &  & 31.99 & 0.312 & 0.537 & 0.16 \\
 &  &  &  & 22.84 & 0.273 & 0.465 & -0.05 \\ \hline
\multirow{3}{*}{\checkmark} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{\checkmark} & \underline{58.81} & \underline{0.427} & \textbf{0.713} & \underline{0.6} \\
 &  &  &  & \underline{32.69} & \underline{0.315} & \underline{0.542} & \underline{0.19} \\
 &  &  &  & 22.72 & \underline{0.276} & 0.466 & \underline{-0.02} \\ \hline
\end{tabular}
